Making the Cut: A Bandit-based Approach to Tiered Interviewing

Given a huge set of applicants, how should a firm allocate sequential resume screenings, phone interviews, and in-person site visits? In a tiered interview process, later stages (e.g., in-person visits) are more informative, but also more expensive than earlier stages (e.g., resume screenings). Using accepted hiring models and the concept of structured interviews, a best practice in human resources, we cast tiered hiring as a combinatorial pure exploration (CPE) problem in the stochastic multi-armed bandit setting. The goal is to select a subset of arms (in our case, applicants) with some combinatorial structure. We present new algorithms in both the probably approximately correct (PAC) and fixed-budget settings that select a near-optimal cohort with provable guarantees. We show via simulations on real data from one of the largest US-based computer science graduate programs that our algorithms make better hiring decisions or use less budget than the status quo.

==> problem.tex <==
\section{Problem Formulation}\label{sec:model}
We represent a set of $n$ applications $A$ as arms $a \in A$. Each arm has a true utility of $u(a)\in[0,1]$, which is unknown. When an arm $a$ is pulled, a reward is pulled from a distribution with mean $u(a)$ and a $\sigma$-sub-Gaussian tail. A user keeps track of an empirical estimate $\hat{u}(a)$ of that underlying utility, and an uncertainty bound $\rad(a)$ around the empirical estimate. This means that $\hat{u}(a)-\rad(a)< u(a) < \hat{u}(a)+\rad(a)$ with some probability. Once arm $a$ is pulled (ex. an application is reviewed or an interview is performed), $\hat{u}(a)$ and $\rad(a)$ are updated. 

In this problem we define a decision class as $\mathcal{M}_K(A)=\{M\subseteq A \bigm| |M|=K\}$. The overall goal is to choose a \emph{cohort}, or subset of arms, of size $K<n$ that maximizes some submodular and monotone objective function $w:\mathbb{R}^n\times M\in\mathcal{M}_K(A)\rightarrow \mathbb{R}$. 
The algorithm makes use of a maximization oracle
\begin{equation}\label{eq:oracle}
\oracle_K(\hat{\mathbf{u}},A)=\argmax_{M\in\mathcal{M}_K}w(\hat{\mathbf{u}},M)
\end{equation}
and the optimal solution to this MAB problem would be $M*=\oracle(\mathbf{u},A)$. In practice however, the true utilities $\mathbf{u}$ are not known.

We propose two different submodular and monotone objective functions to be used in this setting. The first of which is a top-K objective
\begin{equation}
\wtop(\mathbf{u},M)=\sum_{a\in M}u(a)
\end{equation}
where the objective is to pick the $K$ arms with the highest utility.

The second function is a diversity function. Assume that the arms can be partitioned into $q$ groups $P_1,\cdots,P_q$. The diversity function can then be written as
\begin{equation}
\wdiverse(\mathbf{u},M)=\sum_{a \in M}u(a).
\end{equation}
Research has shown that a more diverse workforse produces better products and increases productivity~\citep{Desrochers01:Local,Hunt15:Diversity}.


We define a gap score for each arm. For each arm $a$ that is in the optimal cohort $M^*$, the gap is the difference in combinatorial utility between $M^*$ and the best set without arm $a$. For each arm $a$ that is not in the optimal set $M^*$, the gap is the difference in combinatorial utility between $M^*$ and the best set with arm $a$. Formally the gap is defined as
\begin{equation}\label{eq:gap_score}
\Delta_a=
	\begin{cases}
		w(M^*)-\max_{M | M\in \mathcal{M}_K \wedge a\in M} w(M) ,& \text{if } a\notin M^*\\
		w(M^*)-\max_{M | M\in \mathcal{M}_K \wedge a\notin M} w(M) ,& \text{if } a \in M^*
	\end{cases}
\end{equation}

The gap score serves as a useful signal for problem hardness, which we use in the theoretical analysis. Formally, the hardness of a problem can be defined as the sum of inverse squared gaps:
\begin{equation}\label{eq:hardness}
\mathbf{H}=\sum_{a\in A} \Delta_a^{-2}
\end{equation}

Similar to the working paper by \citet{Schumann17:Diverse} we have different type of arm pulls. A type of pull is defined by a cost $j$ and an information gain $s$. Information gain represents how confident you are that the received reward is close to the true utility. A weak pull is defined as having a cost of 1 and an information gain of 1. A stronger pull with $s>j>1$ receives a reward as if that arm was pulled $s$ times and the given rewards were averaged together while only costing $j$. In other words, a weak arm pull receives a reward pulled from a distribution with a $\sigma$-sub-Gaussian tail and a stronger arm pull receives a reward pulled from a distribution with a $\frac{\sigma}{\sqrt{s}}$-sub-Gaussian tail.

The user defines $m$ pulling stages (interview/review stages) for the given problem. For each stage $i\in m$ the user defines a cost $j_i$ and an information gain $s_i$ for the type of pull being used in that round. During each stage $K_i$ arms move on to the next stage (we cut off $K_{i-1}-K_i$ arms) where $n=K_0>K_1>\cdots>K_{m-1}>K_m=K)$. The user must therefore define $K_i$ for each $i\in[m-1]$. The arms chosen to move on to the next stage are denoted as $A_m\subset A_{m-1} \subset \cdots \subset A_1 \subset A_0 = A$.

